Universal determination of comagnetometer response to spin couplings

We propose and demonstrate a general method to calibrate the frequency-dependent response of self-compensating noble-gas-alkali-metal comagnetometers to arbitrary spin perturbations. This includes magnetic and nonmagnetic perturbations like rotations and exotic spin interactions. The method is based on a fit of the magnetic field response to an analytical model. The frequency-dependent response of the comagnetometer to arbitrary spin perturbations can be inferred using the fit parameters. We demonstrate the effectiveness of this method by comparing the inferred rotation response to an experimental measurement of the rotation response. Our results show that experiments relying on zero-frequency calibration of the comagnetometer response can over- or under-estimate the comagnetometer sensitivity by orders of magnitude over a wide frequency range. Moreover, this discrepancy accumulates over time as operational parameters tend to drift during comagnetometer operation. The demonstrated calibration protocol enables accurate prediction and control of comagnetometer sensitivity to, for example, ultralight bosonic dark-matter fields coupling to electron or nuclear spins as well as accurate monitoring and control of the relevant system parameters.

==> old_bits.tex <==
\newpage
\section{MP:Things below are the old/work in progress things.}
\begin{itemize}
    \item Add more discussion about the features in Fig. 6 (Electron, nuclear resonance, dip in magnetic response, avoided crossing, dip in rotation response at high frequencies)\MP{Done, must be revisited.}
    \item Discuss explicitly what it means to perturb, the electron spin, the neutron spin and the proton spin. \MP{I don't understand that one}
        \item Add row to figure 6 \MP{Done?}
        \item discuss figure 6 and why it is awesome, and also very well and clever executed. \MP{Done?}
        \item comment on all extrema in the plots \MP{Done?}
\end{itemize}

\begin{itemize}
    \item Method summary \MP{Done}
    \item Interpretation of the results in context of comag searches for dark matter \MP{Done}

    \item Way of data validation for GNOME \MP{Done}

    \item More reliable and robust comagnetometer operation including potential stabilization \MP{Done}

    \item Allowing interpretation of searches for dark matter over broader frequency range \MP{Done}

    \item Allowing reliable gyroscope operation
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width = 0.7\linewidth]{images/DC_sensitivity_estimation.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}
\subsection{To-Do}
\begin{itemize}
  \item Figure out the y-axis for the plots. hat is the normalization. Suggestion: make it dB. That requires to make statements about $b_0$ in eq. 14, - DONE
  \item Describe the procedure in a flow chart. Sort out experimental plots. - DONE
  \item The response to exotic field reconstructed added to figure 4. - DONE
  \item Double-check signs in reconstructed plots!
  \item Describe plots in the results/discussion
  \item Discussion plot: how much can go wrong in a realistic example.
\end{itemize}

%========================================================
%\begin{figure*}
%    \centering
%    \includegraphics{images/Plot4-MainResult.pdf}
%    \caption{Frequency response to magnetic and rotation perturbation for three different values of the applied external field $B_z$. First and third columns are below and above compensation point respectively, while the middle column is at compensation point. The magnetic frequency response is fitted for the three scenarios, and its parameter values used to obtain a fit for the rotation frequency response, as plotted in (c). Data follows the fit up to 10\,Hz. Beyond, the noise floor is reached.}
%    \label{fig:main_results}
%\end{figure*}
\subsection{Old to do}
\begin{itemize}
    \item Figure with the flow chart? \MP{Is mentioned in new to do}
    \item The general idea for fitting. \MP{DONE}
    \item The frequency response to the generic perturbation \MP{DONE}
    \item Fitting function \MP{DONE}
    \item Reconstruction function\MP{DONE}
    \item Experimental data used for the presented results (4-s long routine)\MP{DONE}
    \item Calibration results for different detunnings (Fig.~\ref{fig:main_results})\MP{DONE}
    \item Detuning from the fitting vs. real detunning (plot)\MP{DONE}
    \item 0.19489(29) is the weighted mean ratio \MP{???} of the fit result for the amplitude of the rotation pertubation (2\,mm/s rotation) and the magnetic pertubation (10\,mV in B$_x$-channel).
    \item Figure 6: Add exotic field frequency response (1 is enough). Change the color scale to dB (devide by pertubation)
    \item HOMEWORK: AW read everything. Dani: Make a flow chart for the fitting routine. 
    \item Fig 2 needs derivative, too. Time series could also be normalized.
\end{itemize}


%------------Plan----------------
\section{Bullets for the paper}
The comagnetometer works  with a hybridized electro-nuclear spin resonance. It is therefore principally impossible to address individual spin species with magnetic fields. In fact, the comagnetometer is insensitve to low frequency magnetic pertubations. In both contexts, fundamental and applied physics, comagnetometer systems are used, which makes an accurate calibration important. We show:

\begin{itemize}
  \item the frequency response function to purely electronic pertubations
  \item the frequency response function to purely nuclear pertubations.
  \item how to derive both from the details in the frequency transfer function of the system to 
  magnetic fields.
\end{itemize}

Paper plots should be: 
\begin{enumerate}
  \item Experimental setup 
  \item Method description (from time series to FFT fit)
  \item Example time series (Manu's plot 1 plus x sensitivity (for fun))
  \item Main result (multiplot): fitted magnetic FFT to predict the rotation response. Rotation response can be predicted very well.
  \item Main result: Color map (Measure magnetic->Predicted Rotation)
  \item Add-on main result: How awesome is the Bz fit? Or: some parameter extractions.
  \item Add-on main result: fit for orthogonal sensitivity axis
  \item Not performing this method, not understanding the systems parameter can lead to order of magnitude wrong estimations for frequency amplitudes of dark matter or rotations. Concrete comparison to: Romalis data (flat frequency response between 0.01 and 10 Hz (Helium peak at 20 Hz) and NASDUCK
\end{enumerate}

\begin{itemize}
  \item Spin-perturbation (magnetic, light shift, rotation) spectroscopy plot around the compensation point (showing the avoided electro-nuclear crossing in a frequency heat map)
  \item Theory including the reversal of the potassium spin rotation direction.
  \item Relating the responses, such that just one measurement is needed.
\end{itemize}

\section{Points to work on}
\begin{itemize}
  \item Strongest dark matter search machine this frequency range. \MP{addressed}
  \item Arbitrary frequency range measurement. DC to 100 Hz  \MP{addressed}
  \item Sensitive gyroscope for autonomous driving.  \MP{addressed}
  \item Spin memory a la Ofer Firstenberg.  \MP{addressed}
  \item 4\,s calibration protocol for gyroscope and dark matter machines  \MP{addressed}
  \item Find papers that exclude dark matter and use a wrong frequency response and list them. \MP{Better fits into discussion section?}
  \item The He peaks in the noise underestimates the sensitivity if the calibration is done wrong. See Nasduck paper for the wrong results. By more than 1 order of magnitude.  \MP{addressed}
 \item Other couplings are also wrongly estimated, like gaee etc. But also dark photons and what not.... \MP{Better fits into discussion section?}
 \item btw. this machine also has the highest documented damping of nuclear spin evolution \MP{Not sure where is the appropriate place for this information and if it is true.} \EK{I have alluded to it in Sec. \ref{sec:ExpSetup}.} 
 \item The Bz zeroeing mechanisms a la Kornack doesn't match our data. So, there is a good chance, that they are not at $\Delta B_z=0$. \MP{Better fits to the discussion section? I don't think that they worked outside of the comp. point. We just have an offset for some reason. It might be related to the parametric modulation and the cross talk between the axises (related or not related to the parametric modulation). }
 \item This raises another issue, or angle: is the complete frequency analysis less sensitive to misalignment errors and wrong angles \MP{Better fits to the discussion section? }.
 \item We should make a global fit to the rotation response, to match the amplitude ratio (once and for all). Or we fit the curve with the data and the amplitude as a parameter (of each individual trace).\MP{Adressed with the calculation of the velocity based on the parameters of the rotation.}
  \end{itemize}



\section*{Acknowledgements}
\section{OLD TEXT BITs}
\subsection{Some old mess }
 This set of differential equations is solved by the following function:
and can experimentally be measured by either applying an oscillating magnetic field to the system and measure the amplitude and phase of the response and then sweeping the frequency over the full frequency range. Or, by looking at the impulse response of the system. Basically by stimulating all frequencies at the same time and applying a Fourier transform to the time data.  Another way to get the frequency response is to measure the response to a step in magnetic field, which is called the step response, taking the numerical time derivative of the data and Fourier transforming it.
\begin{enumerate}
    \item Repetition of the comag theory
    \item differential equation with discussion
    \item analytical fit function with parameters
    \item Proposed method to extract the rotation/exotic fields frequency response from magnetic field measurements.
\end{enumerate}

Rotating a comagnetometer is equivalent to a nonmagnetic nuclear coupling \AWIns{Electron also sees rotations}. Here,  ``nonmagnetic" coupling means any spin perturbation that couples differently to electron and nuclear magnetic moments than a magnetic field. The time evolution of coupled electron $\mathbf{P^e}$ and nuclear polarisations $\mathbf{P^n}$ in a comagnetometer can be described by a set of coupled Bloch equations \cite{}:

\begin{widetext}
\begin{align*}
           \frac{d \mathbf{P^e}}{d t} =& \mathbf{\Omega}\times\mathbf{P^e}+\frac{1}{q}\gamma_e \mathbf{(B+b_e+}\lambda M^n\mathbf{ P^n)\times P^e}
        %+(1- \frac{1}{q})\gamma_e \mathbf{b_N^{AM}\times P^e}
        +[R_{se}^{en}\mathbf{(P^n-P^e)} +{\mathbf{(s-P^e)}}R_p- {R^e}\mathbf{P^e} ]/{q} \\
            \frac{d \mathbf{P^n}}{d t} =&
            \mathbf{\Omega}\times\mathbf{P^n}+\gamma_n \mathbf{(B+b_N^{NG}+}\lambda M^e\mathbf{ P^e)\times P^n}+ R_{se}^{en}\mathbf{(P^e-P^n)}- R^n\mathbf{P^n},
\label{eq:BHE_1}
\end{align*}
\end{widetext}

\begin{widetext}
\begin{align*}
           \frac{d \mathbf{P^e}}{d t} =&\frac{1}{q}\gamma_e \mathbf{(\frac{\text{q}}{\gamma_e}\Omega+B+b_e+}\lambda M^n\mathbf{ P^n)\times P^e}
        %+(1- \frac{1}{q})\gamma_e \mathbf{b_N^{AM}\times P^e}
        +[R_{se}^{en}\mathbf{(P^n-P^e)} +{\mathbf{(s-P^e)}}R_p- {R^e}\mathbf{P^e} ]/{q} \\
            \frac{d \mathbf{P^n}}{d t} =&
            \mathbf{\Omega}\times\mathbf{P^n}+\gamma_n \mathbf{(B+b_N^{NG}+}\lambda M^e\mathbf{ P^e)\times P^n}+ R_{se}^{en}\mathbf{(P^e-P^n)}- R^n\mathbf{P^n},
\end{align*}
\end{widetext}
The first term is the torque due to an applied rotation vector $\mathbf{\Omega}$


To solve the coupled differential equation we fourier transform this equation set and solve it. The analytical expression for the frequency response for the different pertubations is given by:
\begin{widetext}
\begin{equation}
    \begin{cases}
        \frac{d \mathbf{P^e}}{d t} =& \mathbf{\Omega}\times\mathbf{P^e}+\frac{1}{q}\gamma_e \mathbf{(B+b_e+}\lambda M^n\mathbf{ P^n)\times P^e}
        %+(1- \frac{1}{q})\gamma_e \mathbf{b_N^{AM}\times P^e}
        +[R_{se}^{en}\mathbf{(P^n-P^e)} +{\mathbf{(s-P^e)}}R_p- {R^e}\mathbf{P^e} ]/{q}, \\
        
            \frac{d \mathbf{P^n}}{d t} =&
            \mathbf{\Omega}\times\mathbf{P^n}+\gamma_n \mathbf{(B+b_N^{NG}+}\lambda M^e\mathbf{ P^e)\times P^n}+ R_{se}^{en}\mathbf{(P^e-P^n)}- R^n\mathbf{P^n},
    \end{cases}
\label{eq:BHE_3}
\end{equation}
\end{widetext}
\clearpage
